Urban traffic congestion control: a DeePC change

Urban traffic congestion remains a pressing challenge in our rapidly expanding cities, despite the abundance of available data and the efforts of policymakers. By leveraging behavioral system theory and data-driven control, this paper exploits the DeePC algorithm in the context of urban traffic control performed via dynamic traffic lights. To validate our approach, we consider a high-fidelity case study using the state-of-the-art simulation software package Simulation of Urban MObility (SUMO). Preliminary results indicate that DeePC outperforms existing approaches across various key metrics, including travel time and CO$_2$ emissions, demonstrating its potential for effective traffic management

==> preamble.tex <==
\usepackage{graphicx} % for pdf, bitmapped graphics files
\usepackage{epstopdf} % for eps to pdf conversion of graphics files
\usepackage{psfrag} % for eps to pdf conversion of graphics files
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\let\proof\relax %
\let\endproof\relax %
\usepackage{amsthm} % theorems
\usepackage{thmtools} % theorem tools
\usepackage{dsfont} % math fonts
\usepackage{color} % colors
\usepackage{tabu} % tabulars
\usepackage{hyperref} % hyperlinks 
\usepackage{cleveref} % hyperlinks
\let\labelindent\relax
\usepackage{enumitem}  % lists 
\setlist[itemize,1]{leftmargin=\dimexpr 22pt} % margins for itemized lists
\usepackage{cite} % for citations
\usepackage{microtype} % fix typing issues
\usepackage{enumerate} % lists and for hyperlinks with urls
\usepackage{url} % to fix typing issues, for lists and for hyperlinks with urls
\usepackage{BOONDOX-ds} % fancy mathbb
\usepackage{tikz} % tikz drawing
\usepackage[fulladjust]{marginnote} % margin notes
\usepackage{sectsty} % change font of paragraphs and sections
\paragraphfont{\bfseries\sffamily} % paragraphs in bold
\allsectionsfont{\bfseries\sffamily} % sections in bold
\usepackage{mathdots} % reverse ddots
\usepackage{lipsum} % dummy text 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		Typesetting 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% bold math
\newcommand{\bm}[1] {\textbf{#1}}

% i.e. and e.g.
\newcommand{\ie}{\textit{i.e\@.}}
\newcommand{\eg}{\textit{e.g\@.}}

% IEEE LaTeX style: grouping references
\renewcommand{\citepunct}{\,,\,} 
\renewcommand{\citedash}{\,--\,}    

%% Enumerate environment
\renewcommand{\theenumi}{(\roman{enumi})}
\renewcommand{\labelenumi}{\theenumi}

%% Redefine paragraph for IEEEtran
\makeatletter
\def\@IEEEsectpunct{.\ \,}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{1.5ex plus 1.5ex minus 0.5ex}%
{0ex}{\normalfont\normalsize\itshape}}
\makeatother

%% Notes and margins
\newcommand{\apmargin}[1]{\marginpar{\color{red}\tiny\bf\ttfamily{Alberto:} #1}}
\newcommand{\TODO}[1]{{\color{red}\bf #1 \protect\normalcolor}}

%% Description not in bold
\renewcommand*\descriptionlabel[1]{\hspace\labelsep\normalfont#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%		Theorems 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 

\declaretheorem[style=definition]{theorem}
\declaretheorem[style=definition]{corollary}
\declaretheorem[style=definition]{proposition}
\declaretheorem[style=definition]{lemma}
\declaretheorem[style=definition,qed=$\vartriangle$]{remark}
\declaretheorem[style=definition,qed=$\blacktriangle$]{example}
\declaretheorem[style=definition,numbered=no,qed=$\lrcorner$]{standing assumption}
\declaretheorem[style=definition,qed=$\lrcorner$]{assumption}
\declaretheorem[style=definition,qed=$\lrcorner$]{definition}
\declaretheorem[style=definition,qed=$\lrcorner$]{problem} %numbered=no
\declaretheorem[style=definition,numbered=no]{claim}

\renewcommand\thmcontinues[1]{continued}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%			 	Mathematical symbols 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%   Equations %%%%%%%%%%  
\newcommand {\nn}{\nonumber}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand {\bseq}{\begin{subequations}}
\newcommand {\eseq}{\end{subequations}}
\newcommand {\bma}{\left[}
\newcommand {\ema}{\right]}

%%%%%%%%%%  Sets  %%%%%%%%%%  

\newcommand {\N}{\mathbb{N}} 	% Natural numbers
\newcommand {\Z}{\mathbb{Z}} 	% Integers
\newcommand {\Zge}{\mathbb{Z}_{+}} 	% Non-negative integers
\newcommand {\R}{\mathbb{R}} 	% Real numbers
\newcommand {\Rplus}{\mathbb{R}_{+}} 	% Positive reals
\newcommand {\T}{\mathbb{T}} 	% Time
\newcommand {\W}{\mathbb{W}} 	% Signals
\newcommand {\B}{\mathcal{B}} 	% Behavior
\renewcommand {\L}{\mathcal{L}} 	% Linear behaviors


%%%%%%%%%%   Operators  %%%%%%%%%%  
\newcommand{\closure}{\operatorname{cl}} % closure
\newcommand{\Ker}{\operatorname{ker}} % kernel
\newcommand{\Image}{\operatorname{image}} % image
\newcommand{\rank}{\operatorname{rank}} % rank
\renewcommand{\Re}{\operatorname{Re}} % real part
\renewcommand{\Im}{\operatorname{Im}} % imaginary part
\newcommand{\adj}{\operatorname{adj}} % adjoint
\newcommand{\transpose}{\mathsf{T}} %\prime or {\mathsf{T}} or \top % transpose
\newcommand{\blockdiag}{\operatorname{block-diag}} % block-diagonal
\newcommand{\argmax}[2] {\mathrm{arg}\max_{#1}#2} %argmax
\newcommand{\argmin}[2] {\mathrm{arg}\min_{#1}#2} %argmin
\newcommand{\vectorones}{\vect{1}} % ones
\newcommand{\vectorzeros}[1][]{\vect{0}_{#1}} % zeros
\newcommand{\norm}[1]{\left\lVert#1\right\rVert} % norm
\newcommand{\Span}{\operatorname{span}} % span
\newcommand{\id}{\operatorname{id}} % identity
\newcommand{\col}{\operatorname{col}} % column 
\newcommand{\diag}{\operatorname{diag}} % diagonal
\newcommand{\trace}{\operatorname{trace}} % trace
\newcommand{\vc}{\operatorname{vec}} % vectorization
\newcommand{\spectrum}[1]{{\sigma({#1})}} % spectrum
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu} % overbar
\newcommand\inner[2]{\left\langle #1 \, , #2 \right\rangle} % inner product
\newcommand{\Bell}{\text{\boldmath$\ell$\unboldmath}} % bold \ell

% Colors
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}

\def\bblue{\color{blue}}
\def\eblue{\protect\normalcolor}
\def\bred{\color{red}}
\def\ered{\protect\normalcolor}

